Spice-E : Structural Priors in 3D Diffusion using Cross-Entity Attention

We are witnessing rapid progress in automatically generating and manipulating 3D assets due to the availability of pretrained text-image diffusion models. However, time-consuming optimization procedures are required for synthesizing each sample, hindering their potential for democratizing 3D content creation. Conversely, 3D diffusion models now train on million-scale 3D datasets, yielding high-quality text-conditional 3D samples within seconds. In this work, we present Spice-E - a neural network that adds structural guidance to 3D diffusion models, extending their usage beyond text-conditional generation. At its core, our framework introduces a cross-entity attention mechanism that allows for multiple entities (in particular, paired input and guidance 3D shapes) to interact via their internal representations within the denoising network. We utilize this mechanism for learning task-specific structural priors in 3D diffusion models from auxiliary guidance shapes. We show that our approach supports a variety of applications, including 3D stylization, semantic shape editing and text-conditional abstraction-to-3D, which transforms primitive-based abstractions into highly-expressive shapes. Extensive experiments demonstrate that Spice-E achieves SOTA performance over these tasks while often being considerably faster than alternative methods. Importantly, this is accomplished without tailoring our approach for any specific task.

==> figures/limitations.tex <==
\begin{figure} 
\centering
\jsubfig{\includegraphics[height=2cm, trim={2cm 2cm 2cm 2cm}, clip]{images/limitations/cond_1.png}}{\footnotesize {Guidance}}\hfill
\jsubfig{\includegraphics[height=2cm, trim={2cm 2cm 2cm 2cm}, clip]{images/limitations/out_1.png}}{\footnotesize {\emph{A bowl of fruit next to a book on a tablecloth}}}\hfill
\jsubfig{\includegraphics[height=2cm, trim={2cm 2cm 2cm 2cm}, clip]{images/results/stylization/watermelon.png}}{\footnotesize {\emph{A watermelon}}} \vspace{1.5pt}
\jsubfig{\includegraphics[height=2cm, trim={2cm 2cm 2cm 2cm}, clip]{images/results/stylization/candle.png}}{\footnotesize {\emph{A candle}}}
% \vspace{-5pt}
\caption{\textbf{Limitations}. Above, we present several failure cases. These likely result from incorrect multiple attribute binding (the fruit bowl and the book blending) or insufficient preservation of the guidance structure (carpet on the horse, not below).}
\label{fig:limitations}
\end{figure}

==> figures/results/abstraction/abstraction.tex <==
\begin{figure} %
\centering % [trim={left bottom right top},clip]
\jsubfig{\includegraphics[height=2cm]{images/results/abstraction/dining_chair/cond.png}\includegraphics[height=2cm]{images/results/abstraction/dining_chair/output.png}}{\footnotesize {``Dining chair"}}
\hfill
\jsubfig{\includegraphics[height=2cm]{images/results/abstraction/pine_chair/cond.png}\includegraphics[height=2cm]{images/results/abstraction/pine_chair/output.png}}{\footnotesize {``Pine chair"}}
\\
\jsubfig{\includegraphics[height=2cm]{images/results/abstraction/Easyjet_A320-214/cond.png}\includegraphics[height=2cm]{images/results/abstraction/Easyjet_A320-214/output.png}}{\footnotesize {``Easyjet A320-214"}}
\hfill
\jsubfig{\includegraphics[height=2cm]{images/results/abstraction/warhawk/cond.png}\includegraphics[height=2cm]{images/results/abstraction/warhawk/output.png}}{\footnotesize {``Warhawk"}}
\vspace{2.5pt}
\caption{\textbf{De-Abstraction Results} \gfc{need to caption}.}
\label{fig:abstraction_results}
\end{figure}

==> figures/results/abstraction/multipose.tex <==
\begin{figure} %
\centering
\rotatebox{90}{Condition}
\jsubfig{\includegraphics[height=1.0cm]{images/comparisons/sketch_shape/sketch_shape_wood.png}}{} \hfill
\jsubfig{\includegraphics[height=1.0cm]{images/comparisons/sketch_shape/sketch_shape_santa.png}}{} \hfill
\jsubfig{\includegraphics[height=1.0cm]{images/comparisons/sketch_shape/sketch_shape_donkey.png}}{} \hfill
\jsubfig{\includegraphics[height=1.0cm]{images/comparisons/sketch_shape/sketch_shape_carousel.png}}{} \vspace{1.5pt} 
\\
\rotatebox{90}{\whitetxt{x}``F16"}
\jsubfig{\includegraphics[height=1.0cm]{images/comparisons/text_2_mesh/text_2_mesh_wood.png}}{}\hfill
\jsubfig{\includegraphics[height=1.0cm]{images/comparisons/text_2_mesh/text_2_mesh_santa.png}}{} \hfill
\jsubfig{\includegraphics[height=1.0cm]{images/comparisons/text_2_mesh/text_2_mesh_donkey.png}}{} \hfill
\jsubfig{\includegraphics[height=1.0cm]{images/comparisons/text_2_mesh/text_2_mesh_carousel.png}}{} 
\vspace{5pt} 
\caption{\textbf{De-Abstraction multipose}.
}
\label{fig:comparisons}
\end{figure}


==> figures/results/abstraction/multiprompt_airplane.tex <==
\begin{figure} %
\centering
\jsubfig{\includegraphics[height=2.3cm, trim={3cm 3cm 3cm 3cm}, clip]{images/results/plane/cond_0.png}}{}\hfill
\jsubfig{\includegraphics[height=2.3cm, trim={3cm 3cm 3cm 3cm}, clip]{images/results/plane/spaceship_0.png}}{}\hfill
\jsubfig{\includegraphics[height=2.3cm, trim={3cm 3cm 3cm 3cm}, clip]{images/results/plane/banana_0.png}}{} \vspace{1.5pt}
\\
\jsubfig{\includegraphics[height=2.3cm, trim={3cm 3cm 3cm 3cm}, clip]{images/results/plane/cond_1.png}}{}\hfill
\jsubfig{\includegraphics[height=2.3cm, trim={3cm 3cm 3cm 3cm}, clip]{images/results/plane/spaceship_2.png}}{}\hfill
\jsubfig{\includegraphics[height=2.3cm, trim={3cm 3cm 3cm 3cm}, clip]{images/results/plane/banana_1.png}}{} \vspace{1.5pt}
\\
\jsubfig{\includegraphics[height=2.3cm, trim={3cm 3cm 3cm 3cm}, clip]{images/results/plane/cond_2.png}}{\footnotesize {Guidance}}\hfill
\jsubfig{\includegraphics[height=2.3cm, trim={3cm 3cm 3cm 3cm}, clip]{images/results/plane/spaceship_1.png}}{\footnotesize {\emph{A spaceship}}}\hfill
\jsubfig{\includegraphics[height=2.3cm, trim={3cm 3cm 3cm 3cm}, clip]{images/results/plane/banana_2.png}}{\footnotesize {\emph{An airplane that looks like a banana}}}
\vspace{5pt} 
\caption{\textbf{Primitive-based Shape Conditioning \emph{Airplane} Results}. \gfc{Need to caption}
}
\label{fig:abstraction_multiprompt_airplane}
\end{figure}


==> figures/results/abstraction/multiprompt_table.tex <==
\begin{figure} %
\centering
\jsubfig{\includegraphics[height=2.3cm, trim={7cm 8.5cm 7cm 7cm}, clip]{images/results/table/cond_0_1.png}}{}\hfill
\jsubfig{\includegraphics[height=2.3cm, trim={1cm 2cm 2cm 2cm}, clip]{images/results/table/round_coffee_0.png}}{}\hfill
\jsubfig{\includegraphics[height=2.3cm, trim={1cm 2cm 0.5cm 2cm}, clip]{images/results/table/ping_pong_0.png}}{} \vspace{1.5pt}
\\
\jsubfig{\includegraphics[height=2.3cm, trim={6.5cm 9cm 7cm 6cm}, clip]{images/results/table/cond_1_1.png}}{}\hfill
\jsubfig{\includegraphics[height=2.3cm, trim={1cm 2.5cm 0.5cm 2cm}, clip]{images/results/table/round_coffee_1.png}}{}\hfill
\jsubfig{\includegraphics[height=2.3cm, trim={1.2cm 1cm 0.5cm 1cm}, clip]{images/results/table/ping_pong_1.png}}{} \vspace{1.5pt}
\\
\jsubfig{\includegraphics[height=2.3cm, trim={4cm 8cm 6cm 4cm}, clip]{images/results/table/cond_3.png}}{\footnotesize {Guidance}}\hfill
\jsubfig{\includegraphics[height=2.3cm]{images/results/table/round_coffee_3.png}}{\footnotesize {\emph{A round coffee table}}}\hfill
\jsubfig{\includegraphics[height=2.3cm]{images/results/table/ping_pong_3.png}}{\footnotesize {\emph{A ping pong table}}}
\vspace{-1pt} 
\caption{Text-conditional abstraction-to-3D results for test shapes from the \emph{Table} category. The leftmost column displays the guidance input --- a proxy cuboid-based shape. The remaining columns showcase our results over two different target text prompts. 
}
\label{fig:abstraction_multiprompt_table}
\end{figure}


==> figures/results/stylization/results.tex <==
\begin{figure} 
\centering
\jsubfig{\includegraphics[height=2cm, trim={2cm 2cm 2cm 2cm}, clip]{images/results/stylization/cond_bottle.png}}{\footnotesize {Guidance}}\hfill
\jsubfig{\includegraphics[height=2cm, trim={2cm 2cm 2cm 2cm}, clip]{images/results/stylization/cork_3.png}}{\footnotesize {\emph{A corked bottle}}}\hfill
\jsubfig{\includegraphics[height=2cm, trim={2cm 2cm 2cm 2cm}, clip]{images/results/stylization/bowling.png}}{\footnotesize {\emph{A bowling pin}}} \vspace{1.5pt}
\jsubfig{\includegraphics[height=2cm, trim={2cm 2cm 2cm 2cm}, clip]{images/results/stylization/wine.png}}{\footnotesize {\emph{A wine bottle}}}
\vspace{1.5pt}
\\
\jsubfig{\includegraphics[height=2cm, trim={2cm 2cm 2cm 2cm}, clip]{images/results/stylization/cond_bowl.png}}{\footnotesize {Guidance}}\hfill
\jsubfig{\includegraphics[height=2cm, trim={2cm 2cm 2cm 2cm}, clip]{images/results/stylization/modern.png}}{\footnotesize {\emph{A modern vase}}}\hfill
\jsubfig{\includegraphics[height=2cm, trim={2cm 2cm 2cm 2cm}, clip]{images/results/stylization/watermelon.png}}{\footnotesize {\emph{A watermelon}}} \vspace{1.5pt}
\jsubfig{\includegraphics[height=2cm, trim={2cm 2cm 2cm 2cm}, clip]{images/results/stylization/candle.png}}{\footnotesize {\emph{A candle}}}
% \vspace{-5pt}
\caption{3D stylization results results are shown above. The leftmost column displays the guidance input --- an uncolored 3D asset. The remaining columns showcase how the guidance input is styled according to the target text prompt.}
\label{fig:stylization_results}
\end{figure}

==> figures/temp.tex <==
\begin{figure} %
\centering
\rotatebox{90}{\hspace{-4pt}\footnotesize{\emph{A Warhawk}}}
\rotatebox{90}{\hspace{-4pt}\footnotesize{\emph{}}}
% \vspace{2pt}
\jsubfig{\includegraphics[height=1.7cm, trim={7.0cm 7.0cm 6.0cm 7.0cm}, clip]{images/comparisons/abstraction/warhawk_cond.png}}{}\hfill
\jsubfig{\includegraphics[height=1.7cm, trim={7.0cm 7.0cm 7.0cm 7.0cm}, clip]{images/comparisons/abstraction/sketch_warhawk.png}}{} \hfill
\jsubfig{\includegraphics[height=1.7cm]{images/comparisons/abstraction/fantasia_warhawk.png}}{} \hfill
\jsubfig{\includegraphics[height=1.7cm, trim={2.0cm 2.0cm 2.0cm 2.0cm}, clip]{images/comparisons/abstraction/ours_warhawk.png}}{} \vspace{1.5pt}
\\ \vspace{2pt}
\rotatebox{90}{\hspace{-4pt}\footnotesize{\emph{A SkyJet British}}}
\rotatebox{90}{\hspace{-4pt}\footnotesize{\emph{Aerospace BAe-146}}}
% \vspace{2pt}
\jsubfig{\includegraphics[height=1.7cm, trim={7.0cm 7.0cm 7.0cm 7.0cm}, clip]{images/comparisons/abstraction/plane.png}}{}\hfill
\jsubfig{\includegraphics[height=1.7cm, trim={7.0cm 7.0cm 7.0cm 7.0cm}, clip]{images/comparisons/abstraction/sketch_plane_1.png}}{} \hfill
\jsubfig{\includegraphics[height=1.7cm]{images/comparisons/abstraction/fantasia_plane_1.png}}{} \hfill
\jsubfig{\includegraphics[height=1.7cm, trim={2.0cm 2.0cm 2.0cm 2.0cm}, clip]{images/comparisons/abstraction/ours_plane_1.png}}{} \vspace{1.5pt}
\\ \vspace{2pt}
\rotatebox{90}{\footnotesize{\emph{A Heavy}}}
\rotatebox{90}{\footnotesize{\emph{Fighter Ship}}}
% \vspace{2pt}
\jsubfig{\includegraphics[height=1.7cm, trim={7.0cm 7.0cm 7.0cm 7.0cm}, clip]{images/comparisons/abstraction/cond_plane_3.png}}{}\hfill
\jsubfig{\includegraphics[height=1.7cm, trim={7.0cm 7.0cm 7.0cm 7.0cm}, clip]{images/comparisons/abstraction/sketch_plane_3.png}}{} \hfill
\jsubfig{\includegraphics[height=1.7cm]{images/comparisons/abstraction/fantasia_plane_3.png}}{} \hfill
\jsubfig{\includegraphics[height=1.7cm, trim={2.0cm 2.0cm 2.0cm 2.0cm}, clip]{images/comparisons/abstraction/ours_plane_3.png}}{} \vspace{1.5pt}
\\ \vspace{2pt}
% \emph{A Modern Chair Stainless Steel}\\
% \vspace{2pt}
\rotatebox{90}{\footnotesize{\emph{A USPAS 2020}}}
\rotatebox{90}{\footnotesize{\emph{T-14 Phantom}}}
\jsubfig{\includegraphics[height=1.7cm, trim={7.0cm 7.0cm 7.0cm 7.0cm}, clip]{images/comparisons/abstraction/phantom_cond.png}}{\footnotesize {Guidance}}\hfill
\jsubfig{\includegraphics[height=1.7cm, trim={7.0cm 6.0cm 6.0cm 6.0cm}, clip]{images/comparisons/abstraction/sketch_phantom.png}}{\footnotesize {SketchShape}} \hfill
\jsubfig{\includegraphics[height=1.7cm]{images/comparisons/abstraction/fantasia_phantom.png}}{\footnotesize {Fantasia 3D}}\hfill
\jsubfig{\includegraphics[height=1.7cm, trim={1.0cm 1.0cm 1.0cm 1.0cm}, clip]{images/comparisons/abstraction/ours_phantom.png}}{\footnotesize {Ours}}
\label{fig:temp}
\end{figure}


==> macros.tex <==
\usepackage[dvipsnames]{xcolor}
\usepackage{multirow}
\usepackage{soul}

%Our comments:
\newcommand{\esc}[1]{{\color{red}[\textbf{ES:} #1]}}
\newcommand{\nac}[1]{{\color{blue}[\textbf{NA:} #1]}}
\newcommand{\hec}[1]{{\color{teal}[\textbf{HE:} #1]}}
\newcommand{\gfc}[1]{{\color{violet}[\textbf{GF:} #1]}}
\newcommand{\dgc}[1]{{\color{orange}[\textbf{DG:} #1]}}
\newcommand{\dcc}[1]{{\color{red}[\textbf{Danny:} #1]}}
\newcommand{\noamTODO}[1]{{\color{red}[\textbf{Noam TODO:} #1]}}
\newcommand{\galTODO}[1]{{\color{blue}[\textbf{Gal TODO:} #1]}}

\newcommand{\whitetxt}[1]{{\color{white}#1}\normalfont}
\newcommand{\ignorethis}[1]{}


\newcommand{\new}[1]{{\textcolor{blue}{#1}}}
\newcommand{\old}[1]{{\textcolor{red}{\st{#1}}}}

%Recurring Names
\def\methodName{\texorpdfstring{SPiC$\cdot$E}{SPiC-E}xspace} %removed $\cdot$
\def\shapE{\texorpdfstring{Shap$\cdot$E}{Shap-E}}
\def\appNameTexturing{Texturing }
\def\appNameAbstraction{3D Generation with an Abstract Prior }
\def\appNameShapetalk{Fine-grained 3D editing }

\newcommand{\acronym}{\texorpdfstring{SPiC$\cdot$E}{SPiC-E} (\textbf{S}tructural \textbf{P}riors \textbf{i}n 3D Diffusion Models using \textbf{C}ross-\textbf{E}ntity Attention)\xspace}


\newcommand{\jbox}[2]{
  \fbox{%
  	\begin{minipage}{#1}%
  		\hfill\vspace{#2}%
  	\end{minipage}%
  }}
\newbox\jsavebox
\newcommand{\jsubfig}[2]{%
	\sbox\jsavebox{#1}%
	\parbox[t]{\wd\jsavebox}{\centering\usebox\jsavebox\\#2}%
	}


\newcommand{\sayitt}[3]{{\small\protect\colorlet{col}{#2}\color{col}{} #3}}
\newcommand{\sayit}[3]{{\small\protect\colorlet{col}{#2}\color{col}\colorbox{col!15}{\textsc{#1:}} #3}}
    % \newcommand{\archway}[1]{\sayit{Left}{cyan}{#1}}
    % \newcommand{\facade}[1]{\sayit{Center}{orange}{#1}}
    % \newcommand{\sundial}[1]{\sayit{Right}{teal}{#1}}   
    \newcommand{\archway}[1]{\sayitt{}{cyan}{#1}}
    \newcommand{\facade}[1]{\sayitt{}{orange}{#1}}
    \newcommand{\sundial}[1]{\sayitt{}{teal}{#1}}

\newcommand{\archwaycolor}[1]{{\color{cyan}#1}\normalfont}
\newcommand{\facadecolor}[1]{{\color{orange}#1}\normalfont}
\newcommand{\sundialcolor}[1]{{\color{teal}#1}\normalfont}

==> macros_arxiv.tex <==
% \usepackage[dvipsnames]{xcolor}
% \usepackage{multirow}
\usepackage{soul}
\usepackage{multirow}
\usepackage{xcolor}
\usepackage{xspace}
%Our comments:
\newcommand{\esc}[1]{{\color{red}[\textbf{ES:} #1]}}
\newcommand{\nac}[1]{{\color{blue}[\textbf{NA:} #1]}}
\newcommand{\hec}[1]{{\color{teal}[\textbf{HE:} #1]}}
\newcommand{\gfc}[1]{{\color{violet}[\textbf{GF:} #1]}}
\newcommand{\dgc}[1]{{\color{orange}[\textbf{DG:} #1]}}
\newcommand{\dcc}[1]{{\color{red}[\textbf{Danny:} #1]}}
\newcommand{\noamTODO}[1]{{\color{red}[\textbf{Noam TODO:} #1]}}
\newcommand{\galTODO}[1]{{\color{blue}[\textbf{Gal TODO:} #1]}}

\newcommand{\whitetxt}[1]{{\color{white}#1}\normalfont}
\newcommand{\ignorethis}[1]{}
%\newcommand{\etal}{\textit{et al.}}
\newcommand{\shortcite}[1]{\cite{#1}}


\newcommand{\new}[1]{{\textcolor{blue}{#1}}}
\newcommand{\old}[1]{{\textcolor{red}{\st{#1}}}}

%Recurring Names
\def\methodName{SPiC$\cdot$E\xspace} %removed $\cdot$
\def\shapE{Shap$\cdot$E\xspace}
\def\appNameTexturing{Texturing }
\def\appNameAbstraction{3D Generation with an Abstract Prior }
\def\appNameShapetalk{Fine-grained 3D editing }

\newcommand{\acronym}{SPiC$\cdot$E (\textbf{S}tructural \textbf{P}riors \textbf{i}n 3D Diffusion Models using \textbf{C}ross-\textbf{E}ntity Attention)\xspace}


\newcommand{\jbox}[2]{
  \fbox{%
  	\begin{minipage}{#1}%
  		\hfill\vspace{#2}%
  	\end{minipage}%
  }}
\newbox\jsavebox
\newcommand{\jsubfig}[2]{%
	\sbox\jsavebox{#1}%
	\parbox[t]{\wd\jsavebox}{\centering\usebox\jsavebox\\#2}%
	}


\newcommand{\sayitt}[3]{{\small\protect\colorlet{col}{#2}\color{col}{} #3}}
\newcommand{\sayit}[3]{{\small\protect\colorlet{col}{#2}\color{col}\colorbox{col!15}{\textsc{#1:}} #3}}
    % \newcommand{\archway}[1]{\sayit{Left}{cyan}{#1}}
    % \newcommand{\facade}[1]{\sayit{Center}{orange}{#1}}
    % \newcommand{\sundial}[1]{\sayit{Right}{teal}{#1}}   
    \newcommand{\archway}[1]{\sayitt{}{cyan}{#1}}
    \newcommand{\facade}[1]{\sayitt{}{orange}{#1}}
    \newcommand{\sundial}[1]{\sayitt{}{teal}{#1}}

\newcommand{\archwaycolor}[1]{{\color{cyan}#1}\normalfont}
\newcommand{\facadecolor}[1]{{\color{orange}#1}\normalfont}
\newcommand{\sundialcolor}[1]{{\color{teal}#1}\normalfont}

\newcommand{\Rone}{{\color{brown}\textbf{R1}}}
\newcommand{\Rtwo}{{\color{blue}\textbf{R2}}}
\newcommand{\Rthree}{{\color{violet}\textbf{R3}}}
\newcommand{\Rfour}{{\color{teal}\textbf{R4}}}
\newcommand{\Rfive}{{\color{orange}\textbf{R5}}}


==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}

\usepackage{multicol}

\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/obsolete.tex <==
The self-attention layers receive as input at each timestep $t$ of the denoising process the noised latent code $l_t$. Consider a specific self-attention layer $\mathcal{A}$. The intermediate features of the network at $\mathcal{A}$, denoted $\theta_\mathcal{A}(l_t)$, are first projected to queries $Q_{\theta(l_t)}=W_Q(\theta(l_t))$, keys $K_{\theta(l_t)}=W_K(\theta(l_t))$, and values $V_{\theta(l_t)}=W_V(\theta(l_t))$ through learned linear projections $W_{Q}$, $W_{K}$, $W_{V}$. 

% , yielding:
% \begin{equation}
% M_{(i,j)} = \text{softmax} \left ( \frac{q_{i,j}\cdot K^T}{\sqrt{d}} \right ),
% \end{equation}
% where $M_{(i,j)}$ represents the attention map at position $(i,j)$.

Much like ControlNet \cite{zhang2023adding}, \methodName achieves additional control over the output of a generative model by manipulating the inputs of network blocks within it. By doing so, we keep the original structure of the generative model intact and allow training to start from a position in which plausible (though unconditioned on 3D) samples are generated. When designing the system which takes a 3D prior and injects it to network blocks within the generative model we aim to achieve the following goals:

\begin{itemize}
    \item Allow for interaction between the prior and various intermediate stages of the de-noised latent.

    \item Keep the existing architecture of the generative model intact.

    \item Ensure that when training starts, the outputs of the overall system are identical to those that would have been generated by the original model. 
\end{itemize}

as shown in ControlNet, $\mathcal{Z}$, on $c_{i}$, $c_{conv}=\mathcal{Z}(c_{i})$. We then project $c_{conv}$ through a learned linear projection $W_{Qc}$ such that $Q_{c}=W_{Qc}\cdot c_{conv}$ \hec{is it clear that we're using the queries?}. We also project $l_{i}$ with learned linear projections $W_{Ql}$, $W_{Kl}$, $W_{Vl}$, resulting in $Q_{l}=W_{Ql}\cdot l_{i}$, $K_{l}=W_{Kl}\cdot l_{i}$ and $V_{l}=W_{Vl}\cdot l_{i}$. We sum $Q_{l}$ and $Q_{c}$ to get our \hec{updated} queries for the attention mechanism, $Q_{sum}=Q_{l}+Q_{c}$, and get our output, $l_{out}$ through attention with $Q_{sum}$, $K_{l}$ and $V_{l}$, $l_{out}=Attn(Q_{sum},K_{l},V_{l})$. In this manner , we allow interaction between the prior and the denoised latent by adding the latent 3D prior as input to our Cross Entity Attention Block, and attending between the latent 3D prior and the denoised latent. We achieve this all while keeping the existing architecture of the generative model intact and by applying zero-convolution on the input conditional latent vector we ensure that when training starts the outputs of the overall system are identical to those that would have been generated by the original model.
Figure \ref{fig:architecture_detailed} provides an overview of our Cross Entity Attention Block.

\hec{Intuitively, why do we perform this addition operation over the queries?}


%\methodName uses a 3D prior, $X$, as controlled guidance for a transformer-based 3D diffusion generative model. In order to do so, we seek to encode $X$ into the latent space of the transformer-based 3D diffusion generative model. We leverage Shap$\cdot$E as an encoder for $X$ and also as a transformer-based 3D diffusion generative model. 
%Shap$\cdot$E first trains an encoder to produce implicit representations of a 3D asset, and then trains a diffusion model on the latent representations produced by the encoder. The encoder receives as input both point clouds rendered views of a 3D asset, and outputs a latent representation of the 3D asset which can be linearly projected into the weights of either a NeRF or an SDF. The encoder is pretrained using a NeRF rendering objective and the diffusion model uses the transformer-based diffusion architecture of Point·E.  The latents are sequences of shape 1024×1024 and for our text-conditional generation a single token containing the CLIP text embedding is pre-pended and the timestep embedding is appended. The diffusion model is trained using a simple $L_{2}$ reconstruction loss.

My questions:
(1) are the features psi the same for c and z? No because psi for z is layer dependent and psi for c is constant for each intermediate block.
\hec{ any intuition for justifying the use of the queries? For one I'm pretty sure that's how they do cross attention in 2D (the text features go to the query input). Values made less sense to me because then you don't get interaction between all the layers of the c latent and the z latent.   Deciding between K and Q is harder to justify I guess, but if I had to try Id say something like: "the queries look at every layer in the condition and ask where in the temporary latent do I need a strong affect to emphasize this layer of the condition. Ensuring every layer in the condition is accounted for." Not sure how much sense that makes but I guess that's my take }


With the recent explosion of text guided diffusion models in image generation also came a variety of applications to extend these models to use more than just text as input, allowing for more personalized results. In text to 3D generation diffusion models however, such methods are as of now mostly unexplored \hec{I don't think we can claim that (it's explored for methods that leverage pre-trained text-image Diffusion models for optimizing differentiable 3D representations}.


%The ability to enforce specific 3D structure while transforming objects based on high-level text directives holds immense promise for democratizing 3D content creation, which still requires considerable knowledge of specialized 3D softwares and is extremely time-consuming.


 
%The problem of transforming 3D objects based on high-level directives, such as text prompts, while enforcing its structure is a longstanding goal in computer vision and graphics. 

%The ability to enforce specific 3D structure



\hec{------------}

%We are experiencing growing interests in automating 3D content creation.
%
From the entertainment and gaming industry, to fashion, medicine and the realm of virtual and augmented reality applications, the ability to create and modify existing 3D models is redefining a plethora of businesses, bringing forth a new era of customization and personalization. 
%
The process of tailoring existing template models to suit a particular artistic vision typically entails laborious manual work, carried out by skilled professionals. 
%
Recent advancements in text-to-3D generation hold immense promise for democratizing 3D content creation, allowing for bypassing specialized 3D editing software using just text prompts as input.
% 
However, 




\medskip
\noindent \textbf{Why is it beneficial to operate over 3D Diffusion models?}

\begin{itemize}
    \item what is claimed in ShapE: In contrast to gradient-based optimization techniques which optimize the 3D representation for individual samples -- requiring "expensive optimization procedures" and work that "must be repeated for every sample that is generated", direct generative models "potentially amortize this work by pre-training on a large dataset". They also show this numerically in Table 2 (Latency column: 200 V100-hr vs. 13V100-sec)
    \item in PointE they also mention the "lack of a strong 3D prior" which may result in falling "into a local minima which don't correspond to meaningful or coherent 3D objects".
\end{itemize}

\medskip \noindent \textbf{What can we do?}
\begin{itemize}
    \item Can we tie it to animations, see NeuMesh (https://zju3dv.github.io/neumesh/) which performs various localized edits (but needs an input mesh) for inspiration? A typical use case: Can we manipulate existing 3D objects through pinch-and-drag deformations? (seems relevant especially to stylization and proxy-driven applications) This is related to DragGAN in 2D.
    \item We can transform 3D geometry into new shapes based on high-level text directive and low-level user constraints, allowing for democratizing 3D content generation in reasonable time.
\end{itemize}


%An underlying assumption in our work is that shape conditioning is essential in solving the various tasks our method can perform. We test this claim by ablating our modifications to the Shap$\cdot{}$E framework and comparing our model with the original Shap$\cdot{}$E model finetuned on the appropriate task-specific dataset with textual guidance only, we call this variant \shapE{}$_{\text{FT}}$.
%To validate the use of cross-entity attention, we compare our final model with two alternative variants of adding structural priors into the Shap$\cdot{}$E architecture. 
%The first such variant makes use of the conditional structural prior only during inference, we call this variant SDEdit3D. SDEdit3D uses a \shapE{}$_{\text{FT}}$ model and as inspired by SDEdit \cite{meng2021sdedit}, during inference we add noise to the conditional structural prior and denoise it with a textual prompt. The final variant we ablate against we call ControlNet3D. In this variant we  add ControlNet to the Shap$\cdot{}$E model in a straight forward manner and freeze and clone the original network blocks of Shap$\cdot{}$E. We train ControlNet3D using shape conditioning and use the conditional structural prior as the conditioning vector in the ControlNet architecture.

==> tables/ablations_stylization.tex <==
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccc}
\toprule
 Method & $\text{CLIP}_{Sim}\uparrow$ & $\text{CLIP}_{Dir}\uparrow$ & $\text{GD} \downarrow$\\
\midrule
ControlNet3D  & 0.26 & \textbf{0.01} &  0.02\\
SDEdit3D & \textbf{0.27} & \textbf{0.01} & 0.09 \\ 
\shapE{}$_{\text{FT}}$  & 0.26 & \textbf{0.01} & 0.20 \\ 
Cross-Entity Attention (Ours) & \textbf{0.27} & \textbf{0.01} & \textbf{0.01}\\  
\bottomrule
\end{tabular}
%\\
}
\caption{\textbf{3D Stylization Ablations.} We evaluate the effect of our cross-entity attention mechanism compared to three different baselines: \shapE{}$_{\text{FT}}$, a \shapE{} model finetuned with text guidance only, SDEdit3D a  \shapE{}$_{\text{FT}}$ model, in which during inference noise is added to the condition and ControlNet3D, a \shapE{} model with a ControlNet architecture, over the 3D stylization task. As illustarted above, our cross-entity attention allows for better faithfulness to the input abstract condition than the baseline methods, while maintaining a high fidelity to the input text prompt.}

\label{tab:stylization_ablation}
\end{table}

==> tables/abstraction_comparison_rebuttal.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{3.0pt}
% \def\arraystretch{1.05}
 \def\arraystretch{1.1}
%  \footnotesize
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{llcccc}
\toprule
   & Method  & $\text{CLIP}_{Sim}\uparrow$ & $\text{CLIP}_{Dir} \uparrow$ & $\text{GD} \downarrow$ & Run Time \\ 
    \midrule 
    \multirow{3}{*}{\rotatebox[origin=c]{90}{\emph{Chair}}} & SketchShape & 0.27 & 0.01 & --- & $\sim \text{15 minutes}$\\
    & Fantasia3D & \textbf{0.28} & 0.01 & 0.04 & $\sim \text{30 minutes}$  \\
    & Ours & \textbf{0.28} & 0.02 & \textbf{0.01} & $\textbf{$\sim$ 20 seconds}$ \\
    & \gfc{Ours + GD} & \textbf{0.28} & \textbf{0.04} & 0.02 & $\sim \text{15 minutes}$ \\
    \midrule 
    \multirow{3}{*}{\rotatebox[origin=c]{90}{\emph{Airplane}}} & SketchShape & \textbf{0.27} & 0.02 & --- & $\sim \text{15 minutes}$\\
    & Fantasia3D & \textbf{0.27} & 0.02 & 0.05 & $\sim \text{30 minutes}$  \\
    & Ours & \textbf{0.27} & \textbf{0.04} & \textbf{0.02} & $\textbf{$\sim$ 20 seconds}$ \\
    & \gfc{Ours + GD} & \textbf{0.27} & 0.03 & 0.03 & $\sim \text{15 minutes}$ \\
    \midrule 
    \multirow{3}{*}{\rotatebox[origin=c]{90}{\emph{Table}}} & SketchShape & 0.26 & 0.01 & --- & $\sim \text{15 minutes}$\\
    & Fantasia3D & 0.26 & 0.01 & 0.08 & $\sim \text{30 minutes}$  \\
    & Ours & \textbf{0.28} & \textbf{0.04} & \textbf{0.01} & $\textbf{$\sim$ 20 seconds}$ \\
    & \gfc{Ours + GD} & \textbf{0.28} & \textbf{0.04} & 0.03 & $\sim \text{15 minutes}$
    \midrule 
    \multirow{3}{*}{\rotatebox[origin=c]{90}{Average}} & SketchShape & 0.27 & 0.01 & --- & $\sim \text{15 minutes}$\\
    & Fantasia3D & 0.27 & 0.01 & 0.06 & $\sim \text{30 minutes}$  \\
    & Ours & \textbf{0.28} & 0.03 & \textbf{0.01} & $\textbf{$\sim$ 20 seconds}$ \\
    & \gfc{Ours + GD} & \textbf{0.28} & \textbf{0.04} & 0.03 & $\sim \text{15 minutes}$\\
\bottomrule
\end{tabular}
}
\caption{\textbf{Performance Breakdown for the Text-conditional Abstraction-to-3D Task.} Above we compare the performance of SketchShape~\cite{metzer2023latent} and Fantasia3D~\cite{chen2023fantasia3d} against ours over the three object categories in the text-conditional abstraction-to-3D task. %As illustrated above, our method can more faithfully preserve the input abstract structure, while exhibiting significantly faster inference time. 
Note that GD is not computed for SketchShape as it outputs a NeRF representation.
}
\label{tab:abstraction_comparison_rebuttal}
\end{table}


==> tables/additiona_ablations_stylizations.tex <==
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccc}
\toprule
 Method & $\text{CLIP}_{Sim}\uparrow$ & $\text{CLIP}_{Dir}\uparrow$ & $\text{GD} \downarrow$\\
\midrule
Cross-Entity Attention Condition Queries & 0.24 & 0.001 & 0.03 \\ 
No zero-convolutions & 0.24 & 0.003 & 0.03 \\ 
Cross-Entity Attention Keys  & 0.26 & \textbf{0.01} &  \textbf{0.01}\\
Cross-Entity Attention Values & \textbf{0.27} & \textbf{0.01} & \textbf{0.01} \\ 
Cross-Entity Attention Queries (Ours) & \textbf{0.27} & \textbf{0.01} & \textbf{0.01}\\  
\bottomrule
\end{tabular}
%\\
}
\caption{\textbf{3D Stylization Additional Ablations.} \gfc{Need to caption}}

\label{tab:stylization_additional_ablation}
\end{table}

==> tables/editing_breakdown_supp2.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{5.0pt}
% \def\arraystretch{1.05}
 \def\arraystretch{1.1}
%  \footnotesize
\centering
\resizebox{0.88\linewidth}{!}{
\begin{tabular}{llccccc}
\toprule
   & Method  & LAB$\uparrow$ & GD$\downarrow$ & $l$-GD $\downarrow$ & CD$\downarrow$ & FPD$\downarrow$ \\ 
    \midrule 
    \multirow{2}{*}{\rotatebox[origin=c]{90}{\emph{Chair}}} 
    % & ChangeIt3D & 0.24 & \textbf{0.003} & \textbf{0.009} & \textbf{0.01} & 22.9\\
    % & Ours / a=0.0,b=1.0 & \textbf{0.50} & \textbf{0.12} & \textbf{0.96} & \textbf{0.01} \\
    % & Ours / a=0.25, b=0.75 & 0.42 & 0.31 & 1.24 & 	\textbf{0.01} \\
    & Ours & 0.44 & 0.005 & 0.013 & 	0.04 & 22.5 \\
    & Ours multi-class & 0.39 & 0.015 & 0.013 & 	0.14 & 47.9 \\
    \midrule 
    \multirow{2}{*}{\rotatebox[origin=c]{90}{\emph{Table}}} 
    % & ChangeIt3D & 0.30 & \textbf{0.003} & \textbf{0.009} & \textbf{0.03} & 32.6\\
    % & Ours / a=0.0,b=1.0 & \textbf{0.5} & \textbf{0.09} & 0.93 & \textbf{0.01} \\
    % & Ours / a=0.25, b=0.75 & 0.39 & 0.40 & 	1.17 & 0.03 \\
    & Ours & 0.41 & 0.009 & 0.013 & 0.05 & 32.0 \\
    & Ours multi-class & 0.36 & 0.020 & 0.013 & 0.11 & 78.4 \\
    \midrule 
    \multirow{2}{*}{\rotatebox[origin=c]{90}{\emph{Lamp}}} 
    % & ChangeIt3D & 0.27 & \textbf{0.004} & 	\textbf{0.009} & 0.14 & 138.7 \\
    % & Ours / a=0.0,b=1.0 & \textbf{0.48} & \textbf{0.13} & 1.39 & 	\textbf{0.03} \\
    % & Ours / a=0.25, b=0.75 & 0.41 & 0.28 & 	1.23 & 0.04 \\
    & Ours & 0.47 & 0.005 & 0.016 & 0.08 & 37.3 \\
    & Ours multi-class & 0.40 & 0.017 & 0.017 & 0.16 & 92.6 \\
    \midrule 
    \multirow{2}{*}{\rotatebox[origin=c]{90}{\emph{Avg.}}} 
    % & ChangeIt3D & 0.27 & \textbf{0.003} & \textbf{0.009} & \textbf{0.05} & 53.6 \\
    % & ChangeIt3D paper & 0.35 & 0.33 & \textbf{0.99} & 0.05 \\
    % & Ours / a=0.0,b=1.0 & \textbf{0.49} & \textbf{0.11} & 1.09 & \textbf{0.02} \\
    % & Ours / a=0.25, b=0.75 & 0.40 & 0.33 & 1.21 & 0.03 \\
    & Ours & 0.44 & 0.007 & 0.013 & 0.05 & 29.9 \\ 
    & Ours multi-class & 0.38 & 0.017 & 0.013 & 0.13 & 68.7 \\ 
\bottomrule
\end{tabular}
}
\caption{\textbf{Performance Breakdown for Semantic Shape Editing Task.  } We trained our model across all three classes, adopting a multi-class approach. The findings indicate that our model is capable of multi-class generation.
}
\label{tab:editing_comparison_supp}
\end{table}


==> tables/fantasia3d_comparison.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{3.0pt}
% \def\arraystretch{1.05}
 \def\arraystretch{1.1}
%  \footnotesize
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
   Metric  & Chair & Table & Airplane & Overall \\ 
    \midrule 
    \multicolumn{5}{c}{Abstract-to-3D} \\
    \midrule
    Conveys Text Prompt while & \multirow{2}{*}{62.93\%} & \multirow{2}{*}{91.86\%} & \multirow{2}{*}{61.36\%} & \multirow{2}{*}{71.03\%} \\
    preserving Guidance Shape & & & & \\
    \midrule
    \multicolumn{5}{c}{Stylization} \\
    \midrule
    Conveys Text Prompt while & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{64.83\%} \\
    preserving Guidance Shape & & & & \\
\bottomrule
\end{tabular}
}
\caption{\esc{\textbf{\methodName{} user preference rates compared to Fantasia3D in the Abstract-to-3D and Stylization settings.} The results in this table indicate the percentage of users preferring our results over Fantsia3D in the context of conveying the text prompt while preserving the guidance structure as best as possible across all shape categories. Note that stylization was tested over samples from our stylization test set - a subset of Objaverse which is not split between 'Chair', 'Table' and 'Airplane' categories.}}
\label{tab:fantasia3d_survey}
\end{table}


==> tables/lab_and_cd_table.tex <==
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{llccc}
\toprule
 & Method & $\text{CLIP}_{Sim}\uparrow$ & $\text{CLIP}_{Dir}\uparrow$ & $\text{GD} \downarrow$ \\
 \midrule 
    \multirow{5}{*}{\rotatebox[origin=c]{90}{\emph{Chair}}} & ControlNet3D & \textbf{0.28} & \textbf{0.02} & 0.03 \\
    & SDEdit3D  & \textbf{0.28} & \textbf{0.02} & 0.06 \\ 
    & \shapE{}$_{\text{FT}}$  & \textbf{0.28} & \textbf{0.02} & 0.07 \\ 
    & \esc{CrossOnly}  & 0.25 & 0.01 & 0.03 \\ 
    & Ours & \textbf{0.28} & \textbf{0.02} & \textbf{0.01} \\  
    \midrule 
    \multirow{5}{*}{\rotatebox[origin=c]{90}{\emph{Airplane}}} & ControlNet3D & 0.26 & 0.03 & 0.03 \\
    & SDEdit3D & \textbf{0.27} & \textbf{0.04} & 0.05 \\ 
    & \shapE{}$_{\text{FT}}$  & 0.26 & 0.03 & 0.05 \\ 
    & \esc{CrossOnly}  & 0.25 & 0.03 & 0.03 \\
    & Ours & \textbf{0.27} & \textbf{0.04} & \textbf{0.02} \\    
\bottomrule
\end{tabular}
%\\
}
\caption{\textbf{Performance Breakdown for the Baseline Ablations.} We compare our cross-entity attention mechanism to three baseline methods over the three categories in the text-conditional abstraction-to-3D task. Our proposed mechanism allows for better preserving the input guidance condition, while maintaining a high fidelity to the target text prompt. For additional details on the baselines, see Section 5.2 in the main paper.}
\label{tab:ablations_abstractions}
\end{table}
